Class-Prototype Conditional Diffusion Model with Gradient Projection for Continual Learning

Mitigating catastrophic forgetting is a key hurdle in continual learning. Deep Generative Replay (GR) provides techniques focused on generating samples from prior tasks to enhance the model's memory capabilities using generative AI models ranging from Generative Adversarial Networks (GANs) to the more recent Diffusion Models (DMs). A major issue is the deterioration in the quality of generated data compared to the original, as the generator continuously self-learns from its outputs. This degradation can lead to the potential risk of catastrophic forgetting (CF) occurring in the classifier. To address this, we propose the Gradient Projection Class-Prototype Conditional Diffusion Model (GPPDM), a GR-based approach for continual learning that enhances image quality in generators and thus reduces the CF in classifiers. The cornerstone of GPPDM is a learnable class prototype that captures the core characteristics of images in a given class. This prototype, integrated into the diffusion model's denoising process, ensures the generation of high-quality images of the old tasks, hence reducing the risk of CF in classifiers. Moreover, to further mitigate the CF of diffusion models, we propose a gradient projection technique tailored for the cross-attention layer of diffusion models to maximally maintain and preserve the representations of old task data in the current task as close as possible to their representations when they first arrived. Our empirical studies on diverse datasets demonstrate that our proposed method significantly outperforms existing state-of-the-art models, highlighting its satisfactory ability to preserve image quality and enhance the model's memory retention.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/9_background.tex <==

% \subsection{Deep Generative Replay Continual Learning}
% \label{sec:background:deep_generative_replay_continual_learning}

\subsection{Diffusion Models}\label{sec:background:diffusion_models}
The forward process of DMs involves incrementally adding Gaussian noise to an image until it fully transforms into pure Gaussian noise. Given true data samples $\bx_0 \thicksim q(\bx_0)$, where $q(\bx_0)$ represents the data distribution over $\mathbb{R}^{d}$, the forward process generates a $K$-length sequence of random variables $\bx_1, \bx_2, ..., \bx_K$. Setting $\alpha_{1}=1$ and $\alpha_{k}\downarrow0$, each $\bx_k$ is derived from $\bx_0$ as follows:
\begin{equation} \label{eq:sample_x_k_0}
    \bx_{k}=\sqrt{\bar{\alpha}_{k}}\bx_{0}+\sqrt{1-\bar{\alpha}_{k}}\bm{\epsilon},
\end{equation}
where $\bar{\alpha}_{k}=\prod_{i=1}^{k}\alpha_{i}$ and $\bm{\epsilon}\sim\mathcal{N}\left(\mathbf{0},\mathbf{I}\right)$. 

The reverse process begins with a prior distribution $p(\bx_K) = \mathcal{N}(\bx_K; \mathbf{0},\mathbf{I})$, and then progressively denoise the noisy image $\bx_K$ to generate new data. DDPM \cite{Jonathan2020DDPM} proposes a simplified objective function for training the diffusion model as follows:
\begin{equation}\label{op:simplied_obj_0}
    \min_\theta\mathbb{E}_{k,\bx_0,\bm\epsilon} \left[\lVert \bm\epsilon - \bm\epsilon_{\theta}\left(\bx_{k},k\right)\rVert^2\right],
\end{equation}
where $\bx_k$ is calculated as described in Eq. (\ref{eq:sample_x_k_0}). This optimization problem suggests learning a network $\bm\epsilon_\theta(\bx_k, k)$ to predict the source noise $\bm{\epsilon}\sim\mathcal{N}\left(\mathbf{0},\mathbf{I}\right)$. 

Ultimately, we can employ Langevin dynamics sampling to generate new images from noise. This sampling initiates with $\bx_K \sim \mathcal{N}(\mathbf{0},\mathbf{I})$. The complete sampling process is as follows:
\begin{equation}
    \bx_{k-1} = \frac{1}{\sqrt{\alpha_k}}\left(\bx_k - \frac{1-\alpha_k}{\sqrt{1-\bar{\alpha}_k}}\bm\epsilon_\theta(\bx_k,k)\right)  + \sigma_k \bz,
\end{equation}
where $\sigma_{k}=\sqrt{\sigma_{k}^2} = \sqrt{\frac{(1-\alpha_k)(1-\bar{\alpha}_{k-1})}{1-\bar{\alpha}_{k}}}$, $\bz \sim \mathcal{N}(\mathbf{0},\mathbf{I})$, and $k=K,...,1$.
\subsection{Classifier-free Guidance}\label
{sec:background:classifier_free_guidance}

The classifier-free approach, as proposed in \cite{ho2021classifierfree}, offers a method to train diffusion models without the need for a separate classifier. It involves simultaneous training of a conditional diffusion model and an unconditional one, generally denoted by $\bm\epsilon_\theta(\bx_k,k,y)$, where $y$ represents conditioning information such as the class label of $\bx$. During training, $y$ is randomly chosen to be either the class $m$-th (i.e., $y=m \in \{1, 2, ..., M\}$), or unknown class (i.e., $y=0$). In the sampling phase, $\tilde{\bm\epsilon}_\theta(\bx_k, k, y)$ is utilized for denoising $\bx_K$ to generate images with class information:
\begin{equation} \label{eq:classifier-free}
    \tilde{\bm\epsilon}_\theta(\bx_k, k, y) = w\bm\epsilon_\theta(\bx_k, k, y=m) + (1 - w)\bm\epsilon(\bx_k, k, y = 0),
\end{equation}
where $w \geq 0$ controls the degree to which the conditioning information is used.

